Charmonium contribution to $B \rightarrow K\ell^+\ell^-: testing the factorization approximation on the lattice

We report the current status of a study of charmonium contribution to $B \rightarrow K\ell^+\ell^-$ on the lattice. Our lattice calculation tests the factorization approximation for this contribution. In order to control the problem of the artificial divergence, we focus on the low $q^2$ region with a small b-quark mass. We also take into account the renormalization constants of relevant four-quark operators calculated through the temporal moments. Results suggest a violation of the factorization approximation.

==> Refs.tex <==
%%
%% WinShell 3.3.2.6
%% http://www.winshell.org/
%%

% Strings


% Preamble


% BibTeX Entries
@article{Aaij:2013pta,
      author         = "Aaij, R and others",
      title          = "{Observation of a resonance in $B^+ \to K^+ \mu^+\mu^-$
                        decays at low recoil}",
      collaboration  = "LHCb",
      journal        = "Phys. Rev. Lett.",
      volume         = "111",
      year           = "2013",
      number         = "11",
      pages          = "112003",
      doi            = "10.1103/PhysRevLett.111.112003",
      eprint         = "1307.7595",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "LHCB-PAPER-2013-039, CERN-PH-EP-2013-137",
      SLACcitation   = "%%CITATION = ARXIV:1307.7595;%%"
}

@article{Lyon:2014hpa,
      author         = "Lyon, James and Zwicky, Roman",
      title          = "{Resonances gone topsy turvy - the charm of QCD or new
                        physics in $b \to s \ell^+ \ell^-$?}",
      year           = "2014",
      eprint         = "1406.0566",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "EDINBURGH-14-10, CP3-ORIGINS-2014-021, DIAS-2014-21",
      SLACcitation   = "%%CITATION = ARXIV:1406.0566;%%"
}
%
@article{Neubert:1997uc,
      author         = "Neubert, Matthias and Stech, Berthold",
      title          = "{Nonleptonic weak decays of B mesons}",
      journal        = "Adv. Ser. Direct. High Energy Phys.",
      volume         = "15",
      year           = "1998",
      pages          = "294-344",
      doi            = "10.1142/9789812812667_0004",
      note           = "[,294(1997)]",
      eprint         = "hep-ph/9705292",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "CERN-TH-97-099, CERN-TH-97-99, HD-THEP-97-23",
      SLACcitation   = "%%CITATION = HEP-PH/9705292;%%"
}
%
@article{Christ:2015aha,
      author         = "Christ, N. H. and Feng, X. and Portelli, A. and
                        Sachrajda, C. T.",
      title          = "{Prospects for a lattice computation of rare kaon decay
                        amplitudes: $K\to\pi\ell^+\ell^-$ decays}",
      collaboration  = "RBC, UKQCD",
      journal        = "Phys. Rev.",
      volume         = "D92",
      year           = "2015",
      number         = "9",
      pages          = "094512",
      doi            = "10.1103/PhysRevD.92.094512",
      eprint         = "1507.03094",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      SLACcitation   = "%%CITATION = ARXIV:1507.03094;%%"
}
%
@article{Christ:2016eae,
      author         = "Christ, Norman H. and Feng, Xu and Portelli, Antonin and
                        Sachrajda, Christopher T.",
      title          = "{Prospects for a lattice computation of rare kaon decay
                        amplitudes II $K\to\pi\nu\bar{\nu}$ decays}",
      collaboration  = "RBC, UKQCD",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "11",
      pages          = "114517",
      doi            = "10.1103/PhysRevD.93.114517",
      eprint         = "1605.04442",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      SLACcitation   = "%%CITATION = ARXIV:1605.04442;%%"
}

@article{Brower:2012vk,
      author         = "Brower, Richard C. and Neff, Harmut and Orginos, Kostas",
      title          = "{The M\"obius domain wall fermion algorithm}",
      journal        = "Comput. Phys. Commun.",
      volume         = "220",
      year           = "2017",
      pages          = "1-19",
      doi            = "10.1016/j.cpc.2017.01.024",
      eprint         = "1206.5214",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      reportNumber   = "JLAB-THY-12-1583",
      SLACcitation   = "%%CITATION = ARXIV:1206.5214;%%"
}

@article{Du:2015tda,
      author         = "Du, Daping and El-Khadra, A. X. and Gottlieb, Steven and
                        Kronfeld, A. S. and Laiho, J. and Lunghi, E. and Van de
                        Water, R. S. and Zhou, Ran",
      title          = "{Phenomenology of semileptonic B-meson decays with form
                        factors from lattice QCD}",
      journal        = "Phys. Rev.",
      volume         = "D93",
      year           = "2016",
      number         = "3",
      pages          = "034005",
      doi            = "10.1103/PhysRevD.93.034005",
      eprint         = "1510.02349",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "FERMILAB-PUB-15-425-T, NSF-KITP-15-134",
      SLACcitation   = "%%CITATION = ARXIV:1510.02349;%%"
}

@article{Aaij:2016cbx,
      author         = "Aaij, Roel and others",
      title          = "{Measurement of the phase difference between short- and
                        long-distance amplitudes in the $B^{+}\to
                        K^{+}\mu^{+}\mu^{-}$ decay}",
      collaboration  = "LHCb",
      journal        = "Eur. Phys. J.",
      volume         = "C77",
      year           = "2017",
      number         = "3",
      pages          = "161",
      doi            = "10.1140/epjc/s10052-017-4703-2",
      eprint         = "1612.06764",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ex",
      reportNumber   = "CERN-EP-2016-301, LHCB-PAPER-2016-045",
      SLACcitation   = "%%CITATION = ARXIV:1612.06764;%%"
}

@article{Beneke:2001at,
      author         = "Beneke, M. and Feldmann, T. and Seidel, D.",
      title          = "{Systematic approach to exclusive $B \to  V l^+ l^-$, $V
                        \gamma$ decays}",
      journal        = "Nucl. Phys.",
      volume         = "B612",
      year           = "2001",
      pages          = "25-58",
      doi            = "10.1016/S0550-3213(01)00366-2",
      eprint         = "hep-ph/0106067",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-ph",
      reportNumber   = "PITHA-01-05",
      SLACcitation   = "%%CITATION = HEP-PH/0106067;%%"
}

@article{Boyle:2012ys,
      author         = "Boyle, P. A. and others",
      title          = "{Emerging understanding of the $\Delta I = 1/2$ Rule from
                        Lattice QCD}",
      collaboration  = "RBC, UKQCD",
      journal        = "Phys. Rev. Lett.",
      volume         = "110",
      year           = "2013",
      number         = "15",
      pages          = "152001",
      doi            = "10.1103/PhysRevLett.110.152001",
      eprint         = "1212.1474",
      archivePrefix  = "arXiv",
      primaryClass   = "hep-lat",
      SLACcitation   = "%%CITATION = ARXIV:1212.1474;%%"
}
